Faking Fake News for Real Fake News Detection: Propaganda-loaded Training Data Generation

Despite recent advances in detecting fake news generated by neural models, their results are not readily applicable to effective detection of human-written disinformation. What limits the successful transfer between them is the sizable gap between machine-generated fake news and human-authored ones, including the notable differences in terms of style and underlying intent. With this in mind, we propose a novel framework for generating training examples that are informed by the known styles and strategies of human-authored propaganda. Specifically, we perform self-critical sequence training guided by natural language inference to ensure the validity of the generated articles, while also incorporating propaganda techniques, such as appeal to authority and loaded language. In particular, we create a new training dataset, PropaNews, with 2,256 examples, which we release for future use. Our experimental results show that fake news detectors trained on PropaNews are better at detecting human-written disinformation by 3.62 - 7.69% F1 score on two public datasets.

==> tables/ablation_study.tex <==
\begin{table}[thb]
    \small
    \centering
    {
    \begin{tabular}{lccc}
        \toprule
        
        Variant  & \textsc{Grover} & \textsc{RoBERTa}   \\ \midrule
        
        \datasetname~ & 66.8 ($\pm$2.0) & 66.9 ($\pm$2.1)\\
        ~~ - AA & 64.2 ($\pm$2.1) & 64.8 ($\pm$2.9) \\
        ~~ - LL & 65.6 ($\pm$2.9) & 65.2 ($\pm$1.8)\\
        ~~ - AA \& LL & 63.8 ($\pm$4.8) & 63.8 ($\pm$4.4) \\
        
        \bottomrule
    \end{tabular}
    }
    
    \caption{Accuracy (in \%) on the the \humanwritten~ dataset for different models when trained on different variants of the \datasetname~ training set. AA denotes \textit{appeal to authority}, whereas LL refers to \textit{loaded language}.}
    \label{tab:ablation_study}
    
\end{table}

==> tables/base_model_human_written_performance.tex <==
\begin{table}[thb]
    \small
    \centering
    {
    \begin{tabular}{lcc}
        \toprule
        Training Data & \textsc{Grover-base}  & \textsc{RoBERTa-base}     \\ \midrule
        \grover~  & ($\pm$)& ($\pm$)\\
        \fakeevent~ & ($\pm$) & ($\pm$)\\
        \datasetname~ & ($\pm$)&  ($\pm$) \\
        
        
        \bottomrule
    \end{tabular}
    }
    
    \caption{Accuracy (in \%) on the \humanwritten~ dataset for different models when trained on on different data.}
    \label{tab:attack_table}
    
\end{table}

==> tables/grover_gen_test_set_performance.tex <==
\begin{table}[thb]
    \small
    \centering
    {
    \begin{tabular}{lcc}
        \toprule
        
        Model & Dev Acc. (\%) & Test Acc. (\%)  \\ \midrule
        % \multicolumn{5}{c}{Gold-standard Training Data} \\ \midrule
        
        
        \textsc{Grover-base} & ($\pm$)& ($\pm$)\\
        \textsc{RoBERTa-base} & 67.5 ($\pm$2.4) &68.9 ($\pm$2.0)\\
        \textsc{Grover-large} & ($\pm$) & ($\pm$)\\
        \textsc{RoBERTa-large} & 70.5 ($\pm$0.3)& 69.8 ($\pm$1.1)\\
        
        \bottomrule
    \end{tabular}
    }
    
    \caption{Test and development set performance on the \grover~-generated dataset of different models. We report the mean and standard deviation of four runs.}
    \label{tab:grover_gen_test}
    
\end{table}

==> tables/mauve.tex <==
\begin{table}[h]
    \small
    \centering
    {
    \begin{tabular}{lc}
        \toprule
        
        \textbf{Training data} & \textsc{Mauve} (\%)  \\ \midrule
        
        \textsc{Grover-gen}   & 27.08\\
        \textsc{\datasetname~}  & 33.11 \\
        
        \bottomrule
    \end{tabular}
    
    }
    \caption{The \textsc{Mauve} score between the generated articles in each training dataset and the disinformative articles in the \humanwritten~ dataset. The higher the score, the closer the two distributions.}
    \label{tab:mauve}
    
\end{table}
